Learning Trajectory Preferences for Manipulators via Iterative Improvement

We consider the problem of learning good trajectories for manipulation tasks. This is challenging because the criterion defining a good trajectory varies with users, tasks and environments. In this paper, we propose a co-active online learning framework for teaching robots the preferences of its users for object manipulation tasks. The key novelty of our approach lies in the type of feedback expected from the user: the human user does not need to demonstrate optimal trajectories as training data, but merely needs to iteratively provide trajectories that slightly improve over the trajectory currently proposed by the system. We argue that this co-active preference feedback can be more easily elicited from the user than demonstrations of optimal trajectories, which are often challenging and non-intuitive to provide on high degrees of freedom manipulators. Nevertheless, theoretical regret bounds of our algorithm match the asymptotic rates of optimal trajectory algorithms. We demonstrate the generalizability of our algorithm on a variety of grocery checkout tasks, for whom, the preferences were not only influenced by the object being manipulated but also by the surrounding environment.\footnote{For more details and a demonstration video, visit: \url{http://pr.cs.cornell.edu/coactive}}

==> experiments.tex <==
% !TEX root = writeup.tex

\vspace*{\sectionReduceTop}
\section{Experiments and Results}
\vspace*{\sectionReduceBot}

\iffalse
\begin{wrapfigure}{0}{0.5\textwidth}
\centering
        \includegraphics[width=1.0\linewidth]{../Figs/placing/placing.png}
        \vskip .05in
        \includegraphics[width=1.0\linewidth]{../Figs/inserting/inserting.png}
            \vskip .05in
        \includegraphics[width=1.0\linewidth]{../Figs/pouring/pouring.png}
 \vspace*{\captionReduceTop}
\caption{In our experiments we consider three activities: placing objects (top), inserting objects (middle),
and pouring liquids (bottom).}
 \vspace*{\captionReduceBot}
\label{fig:real-robot}
\end{wrapfigure}
\fi

\header{Task and Activity Set for Evaluation.}
We evaluate our approach on 35 different robotic tasks.  For each task, we train and test on
scenarios with different objects being manipulated, and/or with a different environment.
% the environment, as well as in the activity being performed.  
We considered following three types of activities:\\
% In our terminology, an  activity consists of a set of
% tasks which differ in the environment and the objects being manipulated.
% Furthermore, a collection of activities form a scenario. We consider the following three kinds of
% scenarios:\\
\emph{1) Manipulation centric:} These activities primarily care for the object being manipulated. Hence
the object's properties and the way robot moves it in the environment is more relevant. We consider 
three activities that are frequently encountered by a household robot:
(a) \emph{pick and place}, e.g., moving a glass of water without spilling water, 
(b) \emph{inserting}, e.g., placing pen inside a pen holder or knife inside a knife 
holder, and (c) \emph{pouring}, e.g., moving a bottle and pouring water from it
into a cup.   By changing the objects and environments, we create 12, 4 and 4 tasks 
respectively for each activity.\\
\emph{2) Environment centric:} These activities also care for the interactions of the object
being manipulated with the surrounding objects. Our object-object interaction
features allow the learning algorithm to handle such type of activities.  We consider
two activities:
% experimentally we demonstrate this on activities involving following two interactions: 
(a) \emph{heavy-fragile}, e.g., moving heavy iron box with glass table in vicinity, and 
(b) \emph{liquid-electronic}, e.g., moving a glass of water with a laptop in vicinity. We create 3
tasks for heavy-fragile and 5 for liquid-electronic activity .\\
\emph{3) Human centric:} These activities additionally have a human in the robot's vicinity. We consider activities where a robot manipulates: 
%vicinity. We consider activities where the robot manipulates the following two kinds of objects:
 (a) \emph{sharp-objects}, e.g., moving a knife with a human in vicinity, and (b)
\emph{hot-objects}, e.g., serving a hot drink. We create 2 and 5 tasks
respectively for each activity.



\header{Baseline algorithms.} 
We evaluate the algorithms that learn preferences from online feedback, under two settings:
(a) \emph{untrained}, where the algorithms learn preferences 
for the new task from scratch without observing any previous feedback; 
(b) \emph{pre-trained}, where the algorithms are pre-trained 
on other similar tasks, and then adapt 
to the new task.
We compare the following algorithms:
% We present a new task to the following set of robots:
\begin{itemize}[leftmargin=*]
 \setlength{\itemsep}{-2pt}
 \setlength{\topsep}{-5pt}
  \setlength{\parsep}{0pt}

\item \emph{Geometric}: It plans a single path, independent of the task, using a BiRRT~\citep{Lavalle01} planner.
\item \emph{Manual}:  It plans a single path following certain manually coded task dependent preferences. % e.g., keep a glass of water upright.
\item \emph{TPP}:  This is our algorithm. We evaluate it under both, \emph{untrained} and \emph{pre-trained} settings.
\item \emph{MMP-online}: This is an online implementation of Maximum margin planning (MMP)~\citep{Ratliff06,Ratliff09a}
algorithm. MMP takes the maximum-margin approach
to make an expert's policy better than any other policy, by a margin.
%MMP accepts an expert's policy and takes the maximum-margin structured prediction approach
%to make it better than any other policy, by a margin.
It can be thought of as a special case of our algorithm with $1$-informative feedback.
%The learning setting it use
%used in MMP 
%pose two challenges in adapting it to our experiments: 
Adapting MMP to our experiments pose two challenges (i) we do not have knowledge of optimal
trajectory or demonstrations; and (ii) the state space of the manipulator we consider is too large, and discretizing will make MMP
intractable. We therefore train MMP from online user feedback observed on a set of trajectories. %the same set of trajectories which are presented to TPP. 
Furthermore, the observed feedbacks are treated as optimal. 
At every iteration we train a structural support vector machine (SVM)~\cite{Joachims09} using all previous feedback as training examples. 
The learned weights are used to predict the trajectory scores for the next iteration. Since we learn on a set of trajectories, the argmax operation in 
structural SVM remains tractable.   To quantify closeness of trajectories, we take $l_2$-norm of the differences in their feature representations. We choose the regularization
parameter $C$ for training structural SVM in hindsight, to give an unfair advantage to MMP-online.



\iffalse
In its original form maximum-margin planning (MMP)~\citep{Ratliff06,Ratliff09a} algorithm 
cannot scale to manipulators with large state and action space, such as PR2.
% We use  algorithm to learn preferences. 
We design a variant of MMP where instead of discretizing
the state space, we directly sample trajectories and reveal a close-to-optimal trajectory to the 
algorithm (this is equivalent to user demonstration).
We train this variant of MMP using the preference perceptron algorithm from~\citep{Shivaswamy12}, 
with a difference that instead of observing the user feedback the algorithm leverage the optimal trajectory
it earlier observed. In supplementary material we show this variant of MMP converge to the 
same solution as the original algorithm~\citep{Ratliff09a}. 
Furthermore, MMP algorithm requires the trajectory reward (score function) to decompose over state-action pairs.
To accommodate this, we define a local approximation of our features from section~\ref{sec:features} and train MMP-sample 
on these features.
\fi

\item \emph{Oracle-svm}: This algorithm leverages the expert's labels on trajectories (hence the name \textit{Oracle}) and is trained 
using SVM-rank~\citep{Joachims06} in a batch manner. This algorithm is \emph{not realizable in practice}, as it requires labeling on the large space of trajectories.
We use this only in pre-trained setting and during prediction it just predicts once and does not learn further.

%  on the same set of  tasks as general-trained-robot.  
%It requires absolute expert's labels, instead of merely the preferences derived from 
%them, on the large space of trajectories. Hence it is infeasible in practice.


\end{itemize}

\iffalse
\begin{wrapfigure}{0}{0.5\linewidth}
\centering
\includegraphics[width=0.5\linewidth,height=0.3\linewidth]{../Figs/labelstatistics/labelstatistics}
\caption{Label statistics of the trajectories}
\label{fig:label}
\end{wrapfigure}
\fi

\header{Evaluation metrics.}
In addition to performing a user study (Section~\ref{sec:user-study}), we also designed a dataset
to quantitatively evaluate the performance of our online algorithm. 
An expert labeled 2100 trajectories on a Likert scale of 1-5 (where 5 is the best)
on the basis of subjective 
human preferences. (The features we designed in Section~\ref{sec:learningalgo} were \textbf{not} revealed to the expert.)
Note that these absolute ratings are never provided
to our algorithms and are only used for the quantitative evaluation of different algorithms.
We quantify the quality of a ranked list of trajectories by its normalized
discounted cumulative gain (nDCG)~\citep{Manning08} at positions 1 and 3 and denote them as nDCG@1 and nDCG@3
respectively. While nDCG@1 is a suitable metric for autonomous robots that execute the top ranked
trajectory, nDCG@3 is suitable for scenarios where the robot is supervised
by humans, (e.g., assembly lines).
We also report average nDCG value over a given number of feedback iterations.

In quantitative analysis, only re-ranking feedback is used. Trajectories 
are observed in order of their current predicted scores and the first trajectory that is better than the top ranked
trajectory is provided as feedback.


\begin{figure}
\vskip -.2in
\centering
\begin{tabular}{@{\hskip -.0in}l@{}c@{\hskip -.2in}c@{\hskip -.2in}c@{}}
\raisebox{.5in}{\rotatebox[origin=c]{90}{\scriptsize nDCG@3}}
&
\subfigure[\scriptsize{Same environment, different object.}]{
\includegraphics[width=0.35\linewidth,height=0.21\textwidth]{../Figs/change_obj/averagred_over_all_tasks_ndcg_3_NumFeebacks_20.pdf}
\label{fig:genobj}
}
&
\subfigure[\scriptsize{New Environment, same object.}]{
\includegraphics[width=0.35\linewidth,height=0.21\textwidth]{../Figs/change_env/averagred_over_all_tasks_ndcg_3_NumFeebacks_20.pdf}
\label{fig:genenv}
}

&

\subfigure[\scriptsize{New Environment, different object.}]{
\includegraphics[width=0.35\linewidth,height=0.21\textwidth]{../Figs/change_both/averagred_over_all_tasks_ndcg_3_NumFeebacks_20.pdf}
\label{fig:genenvobj}
}
\end{tabular}
\vspace*{\captionReduceTop}
\vspace*{\captionReduceTop}
\caption{\text{Study of generalization with change in object, environment and both.}
\textcolor{magenta}{Manual}, Oracle-SVM, \textcolor{blue}{Pre-trained MMP-online (---)},
\textcolor{blue}{Untrained MMP-online (-- --)}, \textcolor{red}{ Pre-trained TPP (---)}, \textcolor{red}{ Untrained TPP (-- --)}. }
\vspace*{\captionReduceBot}
\vspace*{\captionReduceBot}
\vspace*{\captionReduceBot}
% \vspace*{\captionReduceBot}
\label{fig:genstudy}
\end{figure}

\vspace*{\subsectionReduceTop}
\vspace*{\subsectionReduceTop}
\subsection{Results}
\vspace*{\subsectionReduceBot}


\label{sec:results}
\header{How well does TPP generalize to new tasks?} To study generalization of preference feedbacks
we evaluate performance of TPP-pre-trained (i.e., \textit{TPP} algorithm under \textit{pre-trained} setting)
 on a set of tasks the algorithm has not seen before.
We study generalization when: (a) only the object being
manipulated changes, e.g., a bowl replaced by a cup or a bottle, (b)
only the surrounding environment changes, e.g., rearranging objects in the
environment or changing the start location of tasks, and (c) and both change.
Figure~\ref{fig:genstudy} shows nDCG@3 plots averaged over tasks for all types of activities.
TPP-pre-trained starts-off with higher nDCG@3 values than TPP-untrained in all three cases. 
Further, as more feedback are provided, performance of both
algorithms improve and they eventually give identical performance. 
We further observe, an expected generalization behavior; generalizing to tasks with both new environment and object is harder than when only 
one of them changes. Moreover, generalizing to new environment is harder than adjusting to changes in object.

\iffalse
(i) generalizing to tasks with both new environment and object being manipulated 
is harder than, when just one of them changes; and (ii) generalizing with only change in object is easier than with only change in environment.
with only change in object is easier than change in environment  
changes the 
The start-off nDCG value of tpp-trained algorithm when both environment and object changes, is slightly less than 
 when just one of them changes. This is because former is a harder problem.
  %This is an expected behaviour since the former is harder problem and for the same reason we plot it till 50 feedbacks.
\fi

\header{How does TPP compare to MMP-online?} MMP-online proceeds by assuming every user feedback as
optimal, and hence over the time  accumulates many contradictory/incorrect training examples. We
can see in Figure~\ref{fig:genstudy}, pre-training MMP-online does not provide much benefit and its
pre-trained and untrained versions starts-off with similar nDCG@3 values and thereon gives similar performance. 
This study also highlights the sensitivity of MMP to sub-optimal feedback.  

%Even though mmp-sample leverage the knowledge 
%of optimal trajectory, under both trained and untrained settings it lacks behind tpp-trained (Figure~\ref{fig:genstudy}). The reason being,
%mmp-sample learns with local trajectory features while tpp use both local and global features. Due to prior knowledge of optimal trajectory 
%mmp-sample doesn't require user feedback. But algorithmically one iteration
%of mmp-sample is equivalent to one feedback for tpp. 

\begin{wraptable}{r}{0.58\linewidth}
\vskip -.15in
\centering
\caption{\textbf{Comparison of different algorithms and study of features in untrained setting.} Table contains average nDCG@1(nDCG@3)
values over 20 rounds of feedbacks.}
\vspace*{\captionReduceBot}
 \resizebox{0.6\textwidth}{!}{
\begin{tabular}{r@{}rrcccc}\cline{2-7}
&&\multirow{2}{*}{Algorithms}&Manipulation &Environment&Human&\multirow{2}{*}{Mean}\\
&&&centric&centric&centric&\\\cline{2-7}
&&Geometric&0.36 (0.54)&0.43 (0.38)&0.36 (0.27)&0.38 (0.40)\\
&&Manual&0.53 (0.55)&0.39 (0.53)&0.40 (0.37)&0.44 (0.48)\\\cline{2-7}
\multirow{4}{*}{\raisebox{.08in}{\rotatebox[origin=c]{90}{TPP}}}&\multirow{4}{*}{\raisebox{.1in}{\rotatebox[origin=c]{90}{Features}}}&Obj-obj interaction&-&0.57 (0.55)&0.53 (0.48)&0.55 (0.53)\\
&&Robot arm config&0.89 (0.87)&0.75 (0.66)&0.64 (0.53)&0.76 (0.69)\\
&&Object trajectory&0.92 (0.91)&0.80 (0.70)&0.71 (0.60)&0.81 (0.74)  \\
&&Object environment&0.92 (0.90)&0.77 (0.68)&0.60 (0.49)&0.76 (0.69) \\\cline{2-7}
%Random&0.85 (0.85)&0.70 (0.66)&0.57 (0.53)&0.71 (0.68)\\
% MMP-sample&0.92 (0.83)&0.73 (0.66)&0.70 (0.61)&0.78 (0.70)\\
&&TPP (all features)&\textbf{0.93 (0.92)}&\textbf{0.85 (0.75)}&\textbf{0.78 (0.66)}&\textbf{0.85 (0.78)}\\
&&MMP-online&0.83 (0.82)&0.42 (0.51)&0.36 (0.33)&0.54 (0.55)\\
\cline{2-7}
\end{tabular}
 }
 \label{tab:algostudy}
\end{wraptable}




\header{How does TPP compare to Oracle-svm?} Oracle-svm starts off with
nDCG@3 values higher than any other algorithm. The reason being, it is pre-trained using expert's
labels on trajectories, and for the same reason it could not be used in practice. 
One could also observe (Figure~\ref{fig:genstudy}), in less than 5 feedback on new task TPP 
improves over Oracle-svm, which is not updated since it requires expert's labels on test set.

% receives more feedbacks on the new
%tasks, it performance improves and it outperforms Oracle-svm. 

\header{How does TPP compare to Manual?} We code some preferences into the planners e.g., keep 
a glass of water upright. However, some preferences are difficult to specify, e.g., not to move heavy objects over fragile 
items. We empirically found (Figure~\ref{fig:genstudy}) the resultant manual algorithm produce poor trajectories with
an average nDCG@3 of 0.48 over all types of activities. 

% \header{How is tpp compared to mmp-online under untrained setting?}





\iffalse
general-trained-robot on set of tasks it has not seen before. We study
generalization when: only the surrounding environment changes i.e. rearranging objects in the
environment or changing the start location of task, only the object being
manipulated changes i.e. a bowl replaced by a cup or a bottle, and both changes.
Figure~\ref{fig:genstudy} shows nDCG@3 plots averaged over tasks of all the scenarios.
In all three cases general-trained-robot starts off with a higher nDCG values than the un-trained new-robot which
receives preference feedbacks for the first time. As more feedbacks are provided performance of both
robots improves and eventually new-robot starts performing as good as the general-trained-robot. The
start off nDCG value of general-trained-robot when both environment and object changes, is slightly less than 
the cases when just one of them changes. This is an expected behaviour since the former is harder problem. 

Trained and untrained versions of mmp-robot receives optimal feedback but still lacks behind
the general-trained-robot receiving a weaker, expected $\alpha$-informative, feedback. The reason
being,
mmp-robot learns with local trajectory features while general-trained-robot learns both with local
and global features. 
Labeled-robot starts off with
a higher nDCG@3 values than any of the robots. The reason being it learns using expert's labels on
trajectories and therefore this robot is unrealizable in practice. 
One could also observe as the general-trained-robot receives more feedbacks on the new tasks it outperforms the labeled-robot.
 The trajectories
produced by manual-robot, for which we specify some of the preferences e.g. keep a glass of water
upright, has the least nDCG values. In our experiments manually specifying the preferences gives, on
average, an nDCG@3 of \todo{XXX}. 
\fi



\header{How helpful are different features?} Table~\ref{tab:algostudy} shows the performance of the TPP algorithm in 
the untrained setting using different features. Individually each feature capture several aspects indicating goodness of trajectories,
 and combined together they give the best performance.
Object trajectory feature capture preferences related to the orientation of the object, which often plays a crucial role is
determining preferences, e.g., moving a glass of water.  Robot arm configuration and object environment feature partly capture preferences, 
by detecting undesirable contorted arm configurations and maintaining safe distance from surrounding surfaces, respectively. 
%Object-object feature perform better than Manual algorithm and it could be augmented with other features to yield expressive features. 
Object-object feature by itself can only learn, for example, to move water away from a laptop, but might still move it with jerks or contorted arms.
This feature can be combined with other features to yield more expressive features. Nevertheless, by itself it performs better than Manual algorithm. 

Table~\ref{tab:algostudy} also compares TPP and MMP-online under untrained setting.
Since MMP-online accumulates, over time, a lot of contradictory training examples, its performance is much below TPP.
On average, geometric and manual algorithms perform worse than TPP and MMP-online.

\iffalse
learn to keep a cup of water away from electronic items but not to keep it upright and move it without jerks. 
can only teach a robot about interaction between objects, e.g. do not move water too 
close to laptop, and not 
 While none of the features alone perform as good as the overall feature,
object trajectory feature appears to be of particular importance. Since goodness of a trajectory often depends on
the orientation of the object being manipulated, e.g. moving a glass of water, which is captured by object trajectory feature. 
Robot arm configuration feature by itself partly capture preferences, since user preferred trajectories are mostly contortion 
free. Object environment feature put more emphasis on maintaining safe distance from surrounding surfaces and smoothness of trajectory,
hence they are also important. 

These features capture orientation of the object 

% The last row contain feature used by the mmp-sample. 
% Object-object
% and mmp-sample features are local in nature while remaining features are calculated over a set of waypoints. Object
% spacial feature contains both object-environment and object-orientation features (defined in
% section~\ref{sec:features}). As one can observe global features, specially the
% spectrogram features, (row 2,3,4)  are of greater importance in capturing human preferences than local features
%  (row 1,6). 
\todo{[To be written.]}
 While object-object feature is important for activity type 2 and
3, it alone cannot learn user preferences. For example, a robot may learn not to move water near
a laptop, but might still move it with jerks or contorted arms. Our overall feature set consistently gives
best performance for all types of activities.  
\fi


  \begin{wrapfigure}{O}{0.4\textwidth}
  \vskip -.35in
\centering
 \includegraphics[width=\linewidth,height=0.6\linewidth]{../Figs/feedback_study/feedback_ndcg_1_NumFeedbacks_30}
\vspace*{\captionReduceTop}
\vspace*{\captionReduceTop}
\vspace*{\captionReduceTop}
\caption{\textbf{Study of re-ranking feedbacks.} }
\vspace*{\captionReduceBot}
\vspace*{\captionReduceBot}
\label{fig:feedback}
\end{wrapfigure} 

					  
						   
\header{How well do variants of re-ranking feedback perform?} We study  
the following variants of re-ranking feedback:\\
\textit{1. Click-one-to-replace-top:} User observes the trajectories in order of their current predicted scores and clicks on the first trajectory
which is better than the top ranked trajectory. We used this feedback in our quantitative analysis.\\
\textit{2. Click-one-from-5:}  Top $5$ trajectories are shown and user clicks on the one he thinks
is the best.\\
% \textit{3. First-incorrect-order:} The user observes the trajectory one at a time and stops when an incorrect
% ordering of neighboring trajectories is discovered. These pair of trajectories are then swapped.\\
\textit{3. Approximate-argmax}: In this feedback, instead of presenting top ranked trajectories, five  random trajectories are selected 
as candidate. The user selects the best trajectory among these 5 candidates.
%This is a variant of our TPP algorithm where instead of presenting the top-ranked trajectories, we present three trajectories selected at random to the user for feedback.
% , instead of presenting the top-ranked trajectories.
This simulate situations when computing an argmax over trajectories is prohibitive and therefore an approximate argmax is performed.
%Through this we demonstrate the performance of TPP under weak feedback conditions.


Figure~\ref{fig:feedback} shows the performance of TPP-untrained receiving different
kinds of feedbacks and averaged over three types of activities. When feedback are more $\alpha$-informative the algorithm requires
fewer of those to learn preferences. In particular, click-one-to-replace-top and click-one-from-5 
feedbacks are the most informative, while approximate-argmax is the least informative
and therefore requires more feedbacks to reach a given nDCG@1 value. 
% Moreover, the
% while receiving first-incorrect-order feedback algorithm continues to show improvement with every feedback
% because there is always a pair of trajectories which is incorrectly ranked, and swapping which guides the algorithm in the direction of user's true utility. 
Since all the feedback is $\alpha$-informative, for
some $\alpha > 0$, eventually TPP-untrained is able to learn the preferences. These empirical
findings are consistent with the regret bounds presented in section~\ref{sec:learningscore}. 


   
  
\iffalse
\begin{table*}
\noindent
\parbox{.5\linewidth}{
\caption{\textbf{Different features vs performance.} Normalized area below nTRS(nDCG@3) 
curve after 20 rounds of feedbacks. }
\vspace*{\captionReduceBot}
\resizebox{\linewidth}{!}{
\begin{tabular}{l@{}rcccc}\\\hline
&Features&Type 1 &Type 2&Type 3&Mean\\\hline
1\; &Object-object interaction&-&0.57 (0.55)&0.53 (0.48)&0.55 (0.53)\\
2\; &Robot arm configuration&0.89 (0.87)&0.75 (0.66)&0.64 (0.53)&0.76 (0.69)\\
3\; &Object trajectory&0.92 (0.91)&0.80 (0.70)&0.71 (0.60)&0.81 (0.74)  \\
4\; &Object environment&0.92 (0.90)&0.77 (0.68)&0.60 (0.49)&0.76 (0.69) \\
% 3&Object spacial configuration&0.91 (0.89)&0.75 (0.66)&0.53 (0.47)&0.73 (0.68)\\
% 4&Spectrogram features&0.93 (0.91)&0.78 (0.69)&0.71 (0.59)&0.80 (0.73)\\
%Everything without spectrogram&0.90(0.88)&0.83(0.72)&0.71(0.60)&0.82(0.73)\\
5\; &All the features&0.93 (0.92)&0.85 (0.75)&0.78 (0.66)&0.85 (0.78)\\
\hline
% 6&\;Max margin planning features&0.89 (0.87)&0.72 (0.67)&0.66 (0.58)&0.76 (0.71)\\
\end{tabular}
\label{tab:feature-study}
}

}
\parbox{.5\linewidth}{
\caption{\textbf{Comparison of different algorithms.} Normalized area below nTRS(nDCG@3) 
curve after 20 rounds of feedbacks.}
\vspace*{\captionReduceBot}
\resizebox{\linewidth}{!}{
\begin{tabular}{rcccc}\\\hline
Algorithms&Type 1 &Type 2&Type 3&Mean\\\hline
Geometric&0.36 (0.54)&0.43 (0.38)&0.36 (0.27)&0.38 (0.40)\\
Manual&0.53 (0.55)&0.39 (0.53)&0.40 (0.37)&0.44 (0.48)\\
%Random&0.85 (0.85)&0.70 (0.66)&0.57 (0.53)&0.71 (0.68)\\
% MMP-sample&0.92 (0.83)&0.73 (0.66)&0.70 (0.61)&0.78 (0.70)\\
\todo{MMP-online}&0.83 (0.82)&0.42 (0.51)&0.36 (0.33)&0.54 (0.55)\\
TPP&0.93 (0.92)&0.85 (0.75)&0.78 (0.66)&0.85 (0.78)\\
\hline
\end{tabular}
}

}

\end{table*}
\fi

\iffalse
\begin{table*}
\caption{\textbf{User study:} (Left) Shows learning statistics for each user. Self and cross scores of the final learned trajectories. 
The numbers inside bracket is standard deviation and outside is 
mean. (Middle) Shows average quality of the learned trajectory after every one-third of total feedbacks. (Right) Bar chart showing the average number of 
feedbacks (re-ranking and interactive) required for each task.  }

\parbox{.35\linewidth}{
%{\scriptsize
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}ccccc}
\hline
\multirow{2}{*}{User}&\# Re-ranking & \# Interactive & \multicolumn{2}{c}{Trajectory Quality}\\
&feedbacks&feedbacks&self&cross\\\hline
1&3.1 (1.3)&2.4 (2.4)&3.5 (1.1) & 3.6 (0.8)\\
2&2.3 (1.1)&1.8 (2.7)&4.1 (0.7) & 4.1 (0.5)\\
\hline
\end{tabular}
}
%}
}
% \begin{wrapfigure}{0}{0.4\textwidth}
% \includegraphics[width=\linewidth,height=0.6\linewidth]{../Figs/user_study/average_user}
\parbox{.32\linewidth}{
\includegraphics[width=1\linewidth,height=1in]{../Figs/user_study/average_user}
}
% \end{wrapfigure}
% \begin{wrapfigure}{0}{0.4\textwidth}
% \includegraphics[width=\linewidth,height=0.6\linewidth]{../Figs/user_study/average_user}
\parbox{.32\linewidth}{
\includegraphics[width=1\linewidth,height=1in]{../Figs/user_study/bar_chart}
% \end{wrapfigure}
}
\label{tab:userstudy}
\end{table*}
\fi

\begin{wraptable}[19]{r}{0.55\textwidth}
% \begin{table}
\centering
\begin{minipage}[t]{.55\textwidth}
\vskip -.25in
\caption{Shows learning statistics for each user. Self and cross scores of the final learned trajectories. 
The number inside bracket is standard deviation.}
\vspace*{\captionReduceBot}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}ccccc}
\hline
\multirow{2}{*}{User}&\# Re-ranking & \# Interactive & \multicolumn{2}{c}{Trajectory Quality}\\
&feedbacks&feedbacks&self&cross\\\hline
1&3.1 (1.3)&2.4 (2.4)&3.5 (1.1) & 3.6 (0.8)\\
2&2.3 (1.1)&1.8 (2.7)&4.1 (0.7) & 4.1 (0.5)\\
\hline
\end{tabular}
}
\vskip .1in
\label{tab:userstudy}
% \end{minipage}
% \begin{minipage}[t]{.45\textwidth}
\centering
\includegraphics[width=0.48\linewidth]{../Figs/user_study/average_user}
\includegraphics[width=0.48\linewidth]{../Figs/user_study/bar_chart}
\captionof{figure}{(Left) Shows average quality of the learned trajectory after every one-third of total feedbacks. (Right) Bar chart showing the average number of 
feedbacks (re-ranking and interactive) required for each task. Task difficulty increases from 1 to 10.}
\label{fig:userplot}
\end{minipage}

% \end{table}
\end{wraptable}

\vspace*{\subsectionReduceTop}
\subsection{User Study in learning trajectories}
\vspace*{\subsectionReduceBot}

\label{sec:user-study}
We perform a user study of our system on a variety tasks of varying difficulty, showing it is practically realizable, and
in untrained setting it learns in few feedbacks. 

\header{Experiment setup:} In this study, two users used our system to train a robot, using re-ranking and interactive feedback, 
in accordance with their preferences. 
A set of 10 tasks of varying difficulty level was presented to them one at a time, and users were instructed to provide feedback until they
were not satisfied with the top ranked trajectory. As a baseline Oracle-svm was trained on related tasks and evaluated on those 10 tasks. 
To quantify the quality of learning, each user also evaluated their own trajectories (self score), 
the trajectories of the other user (cross score), and those predicted by Oracle-svm, on a Likert 
scale of 1-5. Users were not revealed the trainer of the trajectories they were assessing.
\iffalse
In the user study, two users not associated with the project used our learning system, and trained a robot according to their
preferences. For this study, we sampled 10 out of 35 tasks of varying difficulties, and presented them to the user one at a time. At every iteration the user
had an option to either provide a re-ranking feedback, by moving a trajectory higher up in the ranked list, or an interactive feedback, by graphically 
improving one waypoint of the trajectory. The users were instructed 
to provide feedbacks until they are not satisfied with the top ranked trajectory.
 As a baseline we trained Oracle-svm on related tasks and evaluated it on the same 10 tasks. 

After both the users have finished learning, we assess the quality of top learned trajectories after every one-third of the total feedbacks required for training.
For this assessment,  we present each user with the top trajectories learned by them (self score), the other user (cross score) and Oracle-svm, and asked to evaluate
its quality on a Likert scale of 1 -- 5. The user's were not revealed the algorithm used in learning the trajectory. Cross and self score of a user conveys, assessment
of the trajectories learned by the user, by the other user and by the user himself. 
\fi

\header{Analysis:} The correlation in user's self and cross scores, Table~\ref{tab:userstudy}, suggest both users 
shared similar utility functions. Furthermore, on an average a user took 3 re-ranking and 2 interactive feedback to train an untrained robot.
We conjecture, for a high DoF manipulator, re-ranking feedback are easier to provide than interactive -- which requires modifying the manipulator
joint angles.\\
%On average, both use  re-ranking feedback more frequently than interactive feedback. The reason for this is coupled with the ease of use. 
%For a high DoF manipulator, re-ranking is easier than modifying the joint angles. 
\header{Learning curve:} On average, TPP took 5 feedback to improve over Oracle-svm, Figure~\ref{fig:userplot} (Left).
This is consistent with our quantitative analysis in the previous section.\\ 
%outperforms pre-trained Oracle-svm, Table~\ref{tab:userstudy} (middle). These results are consistent with our quantitative
%analysis in previous section. Furthermore, TPP produce better trajectories than randomly producing a single trajectory.
\header{Task difficulty:} A trend of increase in number of interactive feedback with increase in total number of feedback 
was observed, Figure~\ref{fig:userplot} (Right). We conjecture from this, interactive feedback were more informative than re-ranking and user relied more on them for
difficult tasks. 

%requiring more feedback, user relied 
%An expected trend of increase in the number of feedback with task difficulty was observed. 
%observed was, more feedbacks were required to train difficult tasks,   Table~\ref{tab:userstudy} (right).
%Another interesting observation was, for difficult tasks users rely more on interactive feedbacks. We conjecture, interactive feedbacks
%are more informative, thereby helps in quicker learning, than re-ranking but are harder to provide for high DoF manipulator. 

\iffalse
\begin{figure*}[htbp]
\centering
      
    \subfigure[Scene 1]
    {
        \includegraphics[width=0.3\linewidth]{Figs/scene/scene1}
        \label{fig:scene_11}
    }  
    \subfigure[Scene 2]
    {
        \includegraphics[width=0.3\linewidth]{Figs/scene/scene2}
        \label{fig:scene_12}
    }
    \subfigure[Scene 3]
    {
        \includegraphics[width=0.3\linewidth]{Figs/scene/scene3}
        \label{fig:scene_13}
    }
    \subfigure[Scene 4]
    {
        \includegraphics[width=0.3\linewidth]{Figs/scene/scene4}
        \label{fig:scene_14}
    }
    \subfigure[Scene 5]
    {
        \includegraphics[width=0.3\linewidth]{Figs/scene/scene5}
        \label{fig:scene_15}
    }
    \subfigure[Scene 6]
    {
        \includegraphics[width=0.3\linewidth]{Figs/scene/scene6}
        \label{fig:scene_16}
    }
    \subfigure[Scene 7]
    {
        \includegraphics[width=0.3\linewidth]{Figs/scene/scene7}
        \label{fig:scene_17}
    }
    \subfigure[Scene 8]{
        \includegraphics[width=0.3\linewidth]{Figs/scene/scene8}
        \label{fig:scene_18}
    }
    \subfigure[Scene 9]
    {
        \includegraphics[width=0.3\linewidth]{Figs/scene/scene9}
        \label{fig:scene_19}
    }
    \subfigure[Scene 10]
    {
        \includegraphics[width=0.3\linewidth]{Figs/scene/scene10}
        \label{fig:scene_110}
    }
    \subfigure[Scene 11]
    {
        \includegraphics[width=0.3\linewidth]{Figs/scene/scene11}
        \label{fig:scene_111}
    }
    \subfigure[Scene 12]
    {
        \includegraphics[width=0.3\linewidth]{Figs/scene/scene12}
        \label{fig:scene_112}
    }
\caption{Different Scenes.}
\end{figure*}
\fi




\iffalse
% Just describe in text when discussing the results.
\begin{table}
\centering
\caption{Data set statistics}
\begin{tabular}{ccc}\hline
Activity No. & $\#$ Tasks & $\#$ Trajectories\\\hline
1 & 12 & x \\
2 & 4 & x \\
3 & 4 & x\\
4 & 4 & x \\\hline
\end{tabular}
\label{tab:stats}
\end{table}
\fi



